What and Whence 1I/`Oumuamua: A Contact Binary from the Debris of a Young Planetary System?

The first confirmed interstellar interloper in our Solar System, 1I/`Oumuamua, is likely to be a minor body ejected from another star, but its brief flyby and faintness made it difficult to study. Two remarkable properties are its large (up to 2.5 mag) rotational variability and its motion relative to the Sun before encounter. The former suggests an extremely elongated shape (aspect ratio ~10) and the latter an origin from the protoplanetary disk of a young star in a nearby association. Against expectations, it is also not comet-like. 1I/`Oumuamua's variability can also be explained if it is a contact binary composed of near-equilibrium ellipsoidal components and heterogeneous surfaces, i.e. brighter, dust-mantled inner-facing hemispheres and darker, dust-free outer-facing poles. Such shapes are a plausible outcome of radiation, tides and collisions in systems where planets are clearing planetesimal disks. The probability that 1I/`Oumuamua has the same motion as a young (<~100 Myr) stellar association by coincidence is <1%. If it is young, its detection vs. more numerous, older counterparts could be explained as a selection effect due to darkening of surfaces by Galactic cosmic rays and loss of dust. 1I/`Oumuamua's apparent lack of ices can be explained if ejected rocky planetesimals are characteristically smaller and thus far more numerous than their icy counterparts: the Solar System may currently host several such objects captured by the combined gravity of Jupiter and the Sun.

==> comet.tex <==
\obj's lack of detectable cometary activity despite a perihelion of 0.25~AU indicates lack of ices within 1~m of its surface, the predicted penetration depth of the thermal wave.  \citep{Jewitt2017,Fitzsimmons2017} proposed that cosmic rays have depleted this zone of ices and left an organic-rich residual crust.   However, this mechanism would not explain why long-period comets from the Oort Cloud, which have experienced interstellar conditions at $>10,000$~AU for 4.5~Gyr, retain surface ices and exhibit cometary behavior.  Although the amount of mass in condensible ices dominates that of ``rocks" \citep[by about 2:1 for Solar System abundances,][]{Lodders2003}, the relative numbers of planetesimals with and without ices also depend sensitively on the corresponding size distributions.  The size distribution of Oort cloud comets markedly flattens below a size of 2~km and becomes negligible below 500~m \citep{Fernandez2012}.  If the characteristic size for ejected rocky and ice planetesimals were 100~m (`Oumuamua-like) and 1~km (comet-like), respectively, then the relative numbers would be about 250:1.  Differences in size distribution with semimajor axis (and hence ice content) could arise from variation in the lifetime of disk gas, which promotes (re-)aggregation of smaller bodies, or the more rapid growth of protoplanets close to the star that promote excitation, collisions, and fragmentation of remaining planetesimals \citep{Kenyon2012b}.

